A Novel ICD Coding Method Based on Associated and Hierarchical Code Description Distillation

ICD(International Classification of Diseases) coding involves assigning ICD codes to patients visit based on their medical notes. ICD coding is a challenging multilabel text classification problem due to noisy medical document inputs. Recent advancements in automated ICD coding have enhanced performance by integrating additional data and knowledge bases with the encoding of medical notes and codes. However, most of them ignore the code hierarchy, leading to improper code assignments. To address these problems, we propose a novel framework based on associated and hierarchical code description distillation (AHDD) for better code representation learning and avoidance of improper code assignment.we utilize the code description and the hierarchical structure inherent to the ICD codes. Therefore, in this paper, we leverage the code description and the hierarchical structure inherent to the ICD codes. The code description is also applied to aware the attention layer and output layer. Experimental results on the benchmark dataset show the superiority of the proposed framework over several state-of-the-art baselines.

==> section/00_abstract.tex <==
\begin{abstract}
ICD(International Classification of Diseases) coding involves assigning ICD codes to patients visit based on their medical notes. ICD coding is a challenging multilabel text classification problem due to noisy medical document inputs. Recent advancements in automated ICD coding have enhanced performance by integrating additional data and knowledge bases with the encoding of medical notes and codes. However, most of them ignore the code hierarchy, leading to improper code assignments. To address these problems, we propose a novel method based on associated and hierarchical code description distillation (AHDD) for better code representation learning and avoidance of improper code assignment.we utilize the code description and the hierarchical structure inherent to the ICD codes.
Therefore, in this paper, we leverage the code description and the hierarchical structure inherent to the ICD codes. 
The code description is also applied to aware the attention layer and output layer. Experimental results on the benchmark dataset show the superiority of the proposed method over several state-of-the-art baselines.
\end{abstract}

==> section/06_limitation.tex <==
\section{Limitation}
Our proposed AHDD method needs to calculate the  the label-specific representation of the associated and  hierarchical codes’ description to distill the medical note during the training phase, thus we need a little more GPU resources and computational time. However, the need of resource occupancy and time consumption of our approach does not increase during inference. 

Our method is based on code description, a concise text lacking diversity. To futher capture key words related to label description, more external knowledge will be incorporated to promote medical code prediction task.

==> table/ablation_result_other.tex <==
\begin{table*}
\centering
% \usepackage{tabularray}
\begin{tblr}{
  cells = {c},
  cell{1}{1} = {r=2}{},
  cell{1}{2} = {c=2}{},
  cell{1}{4} = {c=2}{},
  cell{1}{6} = {r=2}{},
  vline{2} = {-}{},
  hline{2} = {2-5}{},
  hline{3-4,8-9,13-14,18-19,23-24} = {-}{},
  hline{1,28} = {-}{0.08em},
}
model            & Auc   &       & F1    &       & P@5   \\
                 & Macro & Micro & Macro & Micro &       \\
CAML+AHDD        & 89.1~ & 91.6~ & 56.3~ & 63.1~ & 62.0~ \\
w/o ADD          & 89.0~ & 91.5~ & 56.2~ & 63.1~ & 61.8~ \\
w/o HDD~         & 89.0~ & 91.6~ & 56.2~ & 63.1~ & 62.0~ \\
w/o D-att        & 88.3~ & 90.9~ & 56.0~ & 63.0~ & 61.8~ \\
w/o D-output     & 89.0~ & 91.6~ & 56.1~ & 63.1~ & 61.6~ \\
MultiresCNN+AHDD & 90.7~ & 93.2~ & 61.3~ & 67.6~ & 64.0~ \\
w/o ADD          & 90.7~ & 93.2~ & 60.4~ & 67.5~ & 63.6~ \\
w/o HDD~         & 90.6~ & 93.2~ & 61.2~ & 67.5~ & 63.6~ \\
w/o D-att        & 90.5~ & 93.1~ & 60.8~ & 67.6~ & 63.9~ \\
w/o D-output     & 90.4~ & 93.0~ & 60.7~ & 67.4~ & 63.8~ \\
LAAT+AHDD        & 92.5~ & 94.6~ & 67.8~ & 71.7~ & 67.3~ \\
w/o ADD          & 92.5~ & 94.6~ & 67.8~ & 71.2~ & 67.2~ \\
w/o HDD~         & 92.5~ & 94.6~ & 67.8~ & 71.4~ & 67.2~ \\
w/o D-att        & 92.1~ & 94.2~ & 66.5~ & 70.6~ & 66.3~ \\
w/o D-output     & 92.0~ & 94.1~ & 66.7~ & 70.7~ & 66.0~ \\
Fusion+AHDD      & 91.2~ & 93.2~ & 62.6~ & 68.1~ & 64.4~ \\
w/o ADD          & 91.1~ & 93.2~ & 61.4~ & 67.5~ & 64.3~ \\
w/o HDD~         & 91.1~ & 93.2~ & 62.4~ & 68.0~ & 64.4~ \\
w/o D-att        & 91.0~ & 93.1~ & 62.6~ & 67.9~ & 63.9~ \\
w/o D-output     & 91.0~ & 93.0~ & 62.5~ & 67.9~ & 64.0~ \\
Rare-ICD+AHDD    & 92.1~ & 94.3~ & 65.8~ & 71.3~ & 66.8~ \\
w/o ADD          & 92.1~ & 94.3~ & 64.3~ & 70.3~ & 66.1~ \\
w/o HDD~         & 91.9~ & 94.2~ & 65.2~ & 70.9~ & 66.1~ \\
w/o D-att        & 91.9~ & 94.3~ & 65.1~ & 71.0~ & 66.0~ \\
w/o D-output     & 91.0~ & 94.0~ & 65.5~ & 70.9~ & 66.0~
\end{tblr}
\caption{Ablation results on other methods on the MIMIC-III 50 dataset. }
\label{Table ablation other} 
\end{table*}

==> table/visualization.tex <==
\begin{table}
\centering
\begin{tblr}{
  width = 1.35\linewidth,
  colspec = {Q[942]},
  vlines,
  hline{1,2,3,4} = {1}{},
}
\textbf{Medical Note(Fusion) :} The patient was taken for an ERCP the day after admission, where he was found to have a stone in the common bile duct treated with sphincterotomy and stone extraction. He was treated with broad spectrum antibiotics. Following the ERCP, he then \textcolor{red}{appeared to} bleed from his sphincterotomy. His \textcolor{red}{initial hematocrit} was 40 and it then fell to 25. He received 2 units of \textcolor{red}{transfusion}. He was then stable after that. \\                                                                                         \textbf{Medical Note(Fusion+AHDD):} The patient was taken for an ERCP the day after admission, where he was found to have a stone in the common bile duct treated with sphincterotomy and stone extraction. He was treated with broad spectrum antibiotics. Following the ERCP, he then appeared to \textcolor{blue}{bleed} from his sphincterotomy. \textcolor{blue}{ His initial hematocrit} was 40 and it then fell to 25. He received 2 units of \textcolor{blue}{transfusion}. He was then stable after that.\\
\textbf{ICD-9 code:285.1}(Acute posthemorrhagic anemia)                                                                                                                                                                                                                                                                                                                                                                                                                                             
\end{tblr}
\end{table}
